Investigating the parametric dependence of the impact of two-way coupling on inertial particle settling in turbulence

Tom et al.\ (J.\ Fluid Mech.\ 947, A7, 2022) investigated the impact of two-way coupling (2WC) on particle settling in turbulence. For the limited parameter choices explored, it was found that 2WC substantially enhances particle settling compared to the one-way coupled (1WC) case, even at low mass loading $\Phi_m$. Moreover, contrary to previous claims, it was demonstrated that preferential sweeping remains the mechanism responsible for the particles settling faster than the Stokes settling velocity in 2WC flows. However, crucial questions remain: 1) how small must $\Phi_m$ be for the effects of 2WC on particle settling to be negligible? 2) does the preferential sweeping mechanism remain relevant in 2WC flows as $\Phi_m$ is increased? To answer these, we explore a much broader portion of the parameter space, and our simulations cover cases where the impact of 2WC on the global fluid statistics ranges from negligible to strong. We find that even for $\Phi_m=7.5\times 10^{-3}$, 2WC can noticeably increase the settling for some choices of the Stokes and Froude numbers. We also demonstrate that even when $\Phi_m$ is large enough for the global fluid statistics to be strongly affected by the particles, preferential sweeping is still the mechanism responsible for the enhanced particle settling. The difference between the 1WC and 2WC cases is that, in the latter the particles are not merely swept around the downward-moving side of vortices, but they also drag the fluid with them as they move down.

==> Appendicies/A01_timeaverage.tex <==
 \section{Convergence of time averaged fluid velocity at particle positions}
\label{app_derivation}

==> Sections/Notes.tex <==
\textcolor{red}{Preferential sweeping: $P((u_z(\bm{x}^p(t),t))<0) \cap (Q>0))$, rather than $$\rm{E}[u_z(\bm{x}^p(t),t))<0~|~Q>0].$$ Former calculates contribution to settling speeds, latter suggests, how likely are particles to be in downward moving, strain-dominated regions.}\\
Thus, 
contribution to settling enhancement from rotation-dominated regions, whereas, $B$ represents the contribution from strain-dominated regions.


\begin{enumerate}
    \item For the smallest volume fractions considered, the effect of $St$ and $Fr$ on the $Q^p$ is negligible. (Potential figure: small Phi, constant St, 3 Fr/ constant Fr, 5 St).
    \item Plots of constant Phi, constant Fr, different St. Plots are very much alike. \\
    - for Phi5 1WC: Fr 0.3 -> 3, left tail falls in. right tail right on top, no change.
    - .........2WC: 
    Especially for Fr=0.3 - gravity kills preferential sampling. very less St dependence. 
    \item 
\end{enumerate}
\textbf{Multiple $\Phi$ per plot}
\begin{enumerate}
    \item For $St=2$, decreasing $Fr$ makes tails more distinguishable from one another. spreading out more prominent for 2WC, 1WC all on top of one another.
    \item .... Phi4, Phi5, large -v3 Q values lot less probable than Phi1,2,3 ()
    \item 
    \item Plots of constant Phi, constant Fr, different St. Plots are very much alike. \\
    - for Phi5 1WC: Fr 0.3 -> 3, left tail falls in. right tail right on top, no change.
    - .........2WC: 
    Especially for Fr=0.3 - gravity kills preferential sampling. very less St dependence. 
    \item 
\end{enumerate}

in figure 3, we show the probability density function of Q along particle trajectories for St = particles and for volume fractions. 
we see that with increasing volume fraction the preferential 

%
$$<-------------------------------------------->$$
\textbf{Discuss with Andy}\\
%
\textcolor{blue}{\underline{Point 1:}}
In Sec.(someprevioussection), we introduced the concept of a scale-dependent Reynolds $St_l$, and a cut-off length-scale $l_c=l_c(St)$, such that only scales $l<l(St)$ contribute to settling. the range of scales contributing to settling enhancement increases with increasing $St$. \cite{tom2019}.

\underline{Answer:}
This does not matter as the Re is very small and all the available length scales contribute to settling enhancement. For example, in \cite{tom2019} Page 258 last line, $\ell_c(St=1)=5.4\times 10^4$ and $\ell_c(St=0.05)/\eta \approx 600$, whereas for our simulation, $L_{\rm box}/\eta \simeq 240$!\\
%
\textcolor{blue}{\underline{Point 2:}}
How do we justify the increase in 1WC settling enhancement with $St$ in this case? Because, clearly, the range of scales contributing to the s.v.e is not increasing. Is it that the larger scales are more effective in enhancement? \\

Note that for $St=0.3$ preferential sweeping is stronger than for $St=1.0$ for $Re_\lambda \simeq 398$\\
%
\textcolor{blue}{\underline{Point 3:}}
Should the contribution to settling enhancement from scales larger than integral scale be small? otherwise, this is just a consequnce of forcing etc? \\
%
\textcolor{blue}{\underline{Point 4:}}
Does it not look bad to have incomplete graphs for a given volume fraction?\\
%




Introduction\\
1. {is there limit on how small Phi should be for it to be relevant}\\
2. {Section 2}
3. {have discussion about how small mass loading can be when whilst still being significant, traditionally .... 
might still be significant for settling prob....} \\
4. {importance of preferential sweeping preferential sweeping still important. some regime it is not not as large phi turbulence structure destroyed.} \\
5. {details of parameter sweep}

==> Sections/OldTextFigs.tex <==
%
\begin{figure}
	\centering
	\vspace{0mm}
	{\begin{overpic}
			[trim = 0mm 60mm 0mm 50mm,scale=0.4,clip,tics=20]{Figures/JCI/PDF_Q.pdf}
			\put(47,0){$\mathcal{Q}/2\langle\mathcal{S}^2\rangle$}			
	\end{overpic}}
	\caption{DNS results for $\mathcal{P}(\mathcal{Q})$ for different $St$, and for the 1WC and 2WC cases.}
	\label{PDF_Q}
\end{figure}

\begin{figure}
	\centering
	\vspace{0mm}
			\subfloat[]
	{\begin{overpic}
			[trim = 0mm 60mm 0mm 50mm,scale=0.4,clip,tics=20]{Figures/JCI/U_Q_int.pdf}
			\put(120,-5){$St$}			
			\put(43,60){$A(\alpha_1)/u_\eta$, 1WC}
			\put(43,48){$B(\alpha_1)/u_\eta$, 1WC}			
			\put(43,36){$A(\alpha_1)/u_\eta$, 2WC}
			\put(43,24){$B(\alpha_1)/u_\eta$, 2WC}								
	\end{overpic}}
	\subfloat[]
		{\begin{overpic}
			[trim = 0mm 60mm 0mm 50mm,scale=0.4,clip,tics=20]{Figures/JCI/Ratio_plot.pdf}
			\put(120,-5){$St$}			
			\put(100,159){$B(\alpha_1)/A(\alpha_1)$, 1WC}
			\put(100,146){$B(\alpha_1)/A(\alpha_1)$, 2WC}
			\put(100,135){$B(\alpha_2)/A(\alpha_2)$, 1WC}
			\put(100,123){$B(\alpha_2)/A(\alpha_2)$, 2WC}					
	\end{overpic}}
	\caption{DNS results for (a) $A/u_\eta$ and $B/u_\eta$ and (b) $B/A$ as a function of $St$ and for the 1WC and 2WC cases. In the plots, $\alpha_1=0$ and $\alpha_2=4\langle\mathcal{S}^2\rangle$.}
	\label{u_av_Q}
\end{figure}
\FloatBarrier

\begin{figure}
\centering
\vspace{0mm}			
	{\begin{overpic}
	[trim = 0mm -25mm -55mm -3mm,
	scale=0.2,clip,tics=20]{Figures/JCI/JCI_SGSVel_StDep_SSpF_Fig01.eps}
\put(48,0.5){\large{$St$}}
\put(-7,20){\rotatebox{90}{\large{$-\langle u_z(\bm{x}^p(t),t)\rangle / u_{\eta}$}}}
\put(15,56.5){\large{1WC}}
\put(15,48.5){\large{2WC}}
	\end{overpic}}
\caption{Normalized settling velocity enhancement for the one-way (1WC) and two-way (2WC) coupled cases shown as a function of $St$.}
\label{Unfilt_SGSVel_StDep}
\end{figure}

\begin{figure}
\centering
\vspace{0mm}			
	{\begin{overpic}
	[trim = 0mm -25mm -55mm -3mm,
	scale=0.2,clip,tics=20]{Figures/JCI/JCI_SGSVel_ReDep_SSpF_Fig01.eps}
\put(48,0.5){\large{$Re_{\lambda}$}}
\put(-7,20){\rotatebox{90}{\large{$-\langle u_z(\bm{x}^p(t),t)\rangle / u_{\eta}$}}}
\put(15,56.5){\large{1WC}}
\put(15,48.5){\large{2WC}}
	\end{overpic}}
\caption{Normalized settling velocity enhancement for the one-way (1WC) and two-way (2WC) coupled cases shown as a function of $Re_{\lambda}$.}
\label{Unfilt_SGSVel_ReDep}
\end{figure}

\begin{figure}
\centering
\vspace{0mm}			
	{\begin{overpic}
	[trim = 0mm -25mm -85mm -3mm,
	scale=0.195,clip,tics=20]{Figures/JCI/JCI_SGSVel_StDep_SSpF_Fig03.eps}
\put(48,0.5){\large{$\ell_F / \eta$}}
\put(-8,22){\rotatebox{90}{\Large{$ \frac{ \langle u'_{z}(\bm{x}^p(t),t)\rangle } {\langle u_{z}(\bm{x}^p(t),t)\rangle} $}}}
% \put(88,51.85){\large{$St = 0.3$ 1WC}}
% \put(88,47.05){\large{$St = 0.3$ 2WC}}
% \put(88,42.25){\large{$St = 0.5$ 1WC}}
% \put(88,37.45){\large{$St = 0.5$ 2WC}}
% \put(88,32.65){\large{$St = 0.7$ 1WC}}
% \put(88,27.85){\large{$St = 0.7$ 2WC}}
% \put(88,23.05){\large{$St = 1.0$ 1WC} }
% \put(88,18.25){\large{$St = 1.0$ 2WC}}
% \put(88,13.45){\large{$St = 2.0$ 1WC}}
% \put(88,8.65){\large{$St = 2.0$ 2WC}}
	\end{overpic}}
\caption{Ratio of sub-grid settling velocity enhancement to the `full' settling velocity enhancement for the 1WC (1WC - open symbols, dashed line) and 2WC (2WC - closed symbols, solid line) cases shown as a function of the normalized filtering length $\ell_F/\eta$.}
\label{SGS_by_Unfilt_Vel_StDep_ScaleDep}
\end{figure}

\begin{comment}
\textcolor{magenta}{
\begin{itemize}
    \item Should we briefly summarize why computing $\langle {u'}_{z} \rangle (x^{p}(t),t)$ is appropriate to compare with theory \textcolor{green}{???} \textcolor{magenta}{I meant the first paragraph of Section 3.2 `Testing Methodology' in Tom \& Bragg, 2019}
    \item sharp spectral filter
    \item Averaging for 100 turnover times (Rosa 2016; Also Settling velocity of small inertial particles in homogeneous isotropic turbulence from high-resolution DNS, Rosa et al IJMF 2016)
    \end{itemize}}
\end{comment}

\textcolor{magenta}{Another point Maurizio raised was whether we should comment about the saturation of the 1WC/2WC ratios in these plots and if that would help us to infer the scales up to which 2WC has an effect. Would it be reasonable to claim if we can observe saturation on N = 128, St = 0.3 case in  figure \ref{SGSVel_1WC2WC_ratio_StDep_ScaleDep} and N = 256, St = 1 case in  figure \ref{SGSVel_1WC2WC_ratio_ReDep_ScaleDep}?} \textcolor{red}{In one sense our results show no saturation; 2WC appears to be important at all scales since $\langle{u}_z(\bm{x}^p(t),t)\rangle$ is greater for 2WC than for 1WC at all scales. Perhaps the saturation you are referring to is the saturation of their ratios with increasing $\ell_F$? If so, i'm not sure what the significance of that is; it might just be approaching a constant value simply because $\ell_F$ is approaching the largest scales in the flow (and so the saturation is not really significant).}


==> Sections/WritingPointers.tex <==
\begin{comment}

MINOR POINTS
in figures 6 and 7 "A" and "B" seem not very evocative. Can we describe briefly in the caption what they indicate?
sec 4.4 starts at the end of the page

Ok

INTRODUCTION
Summarize importance of particle settling
discuss previous results (Maxey, Wang and Maxey, explanation on pref sweep)
Experiments gave similar results (2wc by default, but very low volume fraction) 
Most of the experiments observed increasing settling velocity, but there are some observations of decreasing settling vel (Nielsen 1993 first observation of loitering). Only with non linear drag and in peculiar situations for DNS (very rare, see Josin's paper)

Most of the studies for 1wc, but reality is 2wc both theory and practical purposes

Recent studies at higher volume fractions (experimental papers) preferential sweeping is also active in 2wc.

2wc DNSs are not that frequent, especially on the settling enhancement

Monchaux relevant enhancement of setting due to 2wc even at low volume fraction, but the fluid statistics stayed the same more or less

Two mechanisms: preferential sweeping and fluid velocity field modified by the particles (sample a different field)

2019 Josin: two contributions to settling, same discussed in experimental papers.
Aim of the paper: how these two mechanisms are modified at different scales





DNS section

Equations of motion, pressure also modified
Exponential integrators for both fluid and particles
mono-disperse particles
nufft for particle feedback
hipstr and nsp validated against each other, plus nufft validation
mean velocity set to zero for all t, meiburg and monchaux pressure mean gradient balances particles weight
physical justification for this, effect of the ground in the atmosphere, zero mass flux. Leave it to Andy?
Filtering methodology - sharp-spectral filter, interpolating the sub-grid velocities and filtered gradients to particle positions
Table of Re and St
Simonin, Horwitz and Mani, numerical issues on 2wc
.05 is the largest dp/eta for our simulations
Artificial periodicity effects, Fr is large, that's fine
We use Fr=1, we focus on the physical mechanism, not specifically to clouds. The mechanism is independnent of the Froude number. Let Andy check this.
Compared our results from our code and Maurizio code and results match very well




Results

Unfiltered first, two-way coupling enhances
in our range settling up with St and Re
how magnitude of enhancement compares 2017PRF, 2006Bosse, 2021Rosa (underestimated enhancement, may be numerical interpolation or computational particles and/or averaging times) enhancement depends on scale separation, different even if Re are relatively similar. Qualitatively same, quant not
fig 3,4 small scales are very effective in 2wc (fluid drag mech)
Despite that (10^3 enhancement) we don't as a large effect compared to that at the small scales (probably small energy of the small scales)
Q results: pref sampl reduces with 2wc so that's not the reason why settling increases. So it should be the fluid drag.
At small scales fluid velocity at part has large energy.


Josin Comments:
This can be attributed to the fluid drag mechanism, where particles drag the surrounding fluid down with them as they fall down under the influence of gravity. The effect of two-way coupling decreases with increasing scale. This could be explained by the effectiveness of particles to pull eddies of different sizes. 

According to Kolmogorovs's 1941 theory, K41 \cite{pope}, the size and energy associated with an eddy increases with increasing scales. Hence the fluid-drag mechanism would be effective at larger scales as they would be more effective in pulling down eddies of comparable energy. Particles can pull eddies down with them, but the larger eddies would be affected less than smaller eddies.

\textcolor{magenta}{Should we mention that 2WC (and even enhancement due to preferential sweeping) is traditionally ignored in weather forecasting models, but the finding in the PRF paper implies that these models might be under predicting settling velocities etc.? Or is it more appropriate in the conclusions section?}

\end{comment}

\begin{comment}

\begin{figure}
\centering
\vspace{0mm}			
	{\begin{overpic}
	[trim = 0mm -25mm -82mm -3mm,
	scale=0.2,clip,tics=20]{Figures/JCI/JCI_EnSpec_StDep_Fig01.eps}
\put(48,2){\large{$\kappa$}}
\put(-5,28){\rotatebox{90}{\large{$E(\kappa)$}}}		
\put(88.5,51.85){\large{$St = 0.3$ 1WC}}
\put(88.5,47.05){\large{$St = 0.3$ 2WC}}
\put(88.5,42.25){\large{$St = 0.5$ 1WC}}
\put(88.5,37.45){\large{$St = 0.5$ 2WC}}
\put(88.5,32.65){\large{$St = 0.7$ 1WC}}
\put(88.5,27.85){\large{$St = 0.7$ 2WC}}
\put(88.5,23.05){\large{$St = 1.0$ 1WC} }
\put(88.5,18.25){\large{$St = 1.0$ 2WC}}
\put(88.5,13.45){\large{$St = 2.0$ 1WC}}
\put(88.5,8.65){\large{$St = 2.0$ 2WC}}
\put(6,10){
\begin{overpic}[trim = 0mm 0mm 0mm 0mm, scale=0.1,clip,tics=20]
{Figures/JCI/JCI_EnSpec_StDep_Fig02.eps}
\end{overpic}
}
	\end{overpic}}
\caption{Ratio of one-way coupled (1WC) sub-grid settling velocity enhancement to that of the two-way coupled (2WC) case shown as a function of the normalized filtering length $\ell_F/\eta$.}
\label{EnSpec_StDep}
\end{figure}

\end{comment}
